Convective-reactive nucleosynthesis of K, Sc, Cl and p-process isotopes in O-C shell mergers

We address the deficiency of odd-Z elements P, Cl, K and Sc in galactic chemical evolution models through an investigation of the nucleosynthesis of interacting convective O- and C shells in massive stars. 3D hydrodynamic simulations of O-shell convection with moderate C-ingestion rates show no dramatic deviation from spherical symmetry. We derive a spherically averaged diffusion coefficient for 1D nucleosynthesis simulations which show that such convective-reactive ingestion events can be a production site for P, Cl, K and Sc. An entrainment rate of $10^{-3}{{\rm M}_\odot}$/s features overproduction factors $OP_\mathrm{s} \approx 7$. Full O-C shell mergers in our 1D stellar evolution massive star models have overproduction factors $OP_\mathrm{m}>1 \mathrm{dex}$ but for such cases 3D hydrodynamic simulations suggest deviations from spherical symmetry. p-process species can be produced with overproduction factors of $OP_\mathrm{m}>1 \mathrm{dex}$, e.g. for $^{130,132}Ba$. Using the uncertain prediction of the $15{{\rm M}_\odot}$, $Z=0.02$ massive star model ($OP_\mathrm{m} \approx 15$) as representative for merger or entrainment convective-reactive events involving O- and C-burning shells, and assume that such events occur in more than 50% of all stars, our chemical evolution models reproduce the observed Galactic trends of the odd-Z elements.

==> abbrev.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Latex abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Equations
\newcommand{\eqt}[1]{Eq.\,(\ref{#1})}
\newcommand{\eqp}[1]{(Eq.\,\ref{#1})}

% Chapters
\newcommand{\sect}[1]{Sect.\,\ref{#1}}

% Figures
\newcommand{\fig}[1]{Fig.\,\ref{#1}}

% Tables
\newcommand{\tab}[1]{Table\,\ref{#1}}

% phrases
\newcommand{\setext}{set\,1\, extension}
\newcommand{\seto}{set\,1}

\newcommand{\mimf}{\mbox{$M_{\rm i}$-$M_{\rm f}$-relation}}
\newcommand{\ms}{main sequence}
\newcommand{\pdcz}{pulse-driven convective zone}

\newcommand{\setopo}{set\,1.1}
\newcommand{\setopt}{set\,1.2}


\newcommand{\spr}{\mbox{$s$-process}}
\newcommand{\sprn}{\mbox{$s$ process}}
\newcommand{\ipr}{\mbox{$i$-process}}
\newcommand{\iprn}{\mbox{$i$ process}}
\newcommand{\npr}{\mbox{$n$-process}}
\newcommand{\nprn}{\mbox{$n$ process}}
\newcommand{\rpr}{\mbox{$r$-process}}
\newcommand{\rprn}{\mbox{$r$ process}}
\newcommand{\ppr}{\mbox{$p$-process}}
\newcommand{\pprn}{\mbox{$p$ process}}


%
%   elements
%
\newcommand{\n}{\ensuremath{\mem{n}}}
\newcommand{\lei}{\ensuremath{^{1}\mem{L}}}
\newcommand{\p}{\ensuremath{\mem{p}}}
\newcommand{\e}{\ensuremath{\mem{e}}}
\newcommand{\epl}{\ensuremath{\mem{e}^\mem{+}}}
\newcommand{\emi}{\ensuremath{\mem{e}^\mem{-}}}
\newcommand{\deu}{\ensuremath{\mem{D}}}
\newcommand{\h}{\ensuremath{\mem{H}}}
\newcommand{\hedr}{\ensuremath{^{3}\mem{He}}}
\newcommand{\hevi}{\ensuremath{^{4}\mem{He}}}
\newcommand{\lisi}{\ensuremath{^{7}\mem{Li}}}
\newcommand{\besi}{\ensuremath{^{7}\mem{Be}}}
\newcommand{\beac}{\ensuremath{^{8}\mem{Be}}}
\newcommand{\bac}{\ensuremath{^{8}\mem{B}}}
\newcommand{\bel}{\ensuremath{^{11}\mem{B}}}
\newcommand{\cdr}{\ensuremath{^{13}\mem{C}}}
\newcommand{\czw}{\ensuremath{^{12}\mem{C}}}
\newcommand{\cel}{\ensuremath{^{11}\mem{C}}}
\newcommand{\cvi}{\ensuremath{^{14}\mem{C}}}
\newcommand{\ndr}{\ensuremath{^{13}\mem{N}}}
\newcommand{\nvi}{\ensuremath{^{14}\mem{N}}}
\newcommand{\nfu}{\ensuremath{^{15}\mem{N}}}
\newcommand{\ovi}{\ensuremath{^{14}\mem{O}}}
\newcommand{\ofu}{\ensuremath{^{15}\mem{O}}}
\newcommand{\ose}{\ensuremath{^{16}\mem{O}}}
\newcommand{\osi}{\ensuremath{^{17}\mem{O}}}
\newcommand{\oac}{\ensuremath{^{18}\mem{O}}}
\newcommand{\fsi}{\ensuremath{^{17}\mem{F}}}
\newcommand{\fac}{\ensuremath{^{18}\mem{F}}}
\newcommand{\fne}{\ensuremath{^{19}\mem{F}}}
\newcommand{\nezwa}{\ensuremath{^{20}\mem{Ne}}}
\newcommand{\neei}{\ensuremath{^{21}\mem{Ne}}}
\newcommand{\nezw}{\ensuremath{^{22}\mem{Ne}}}
\newcommand{\naei}{\ensuremath{^{21}\mem{Na}}}
\newcommand{\nazw}{\ensuremath{^{22}\mem{Na}}}
\newcommand{\nadr}{\ensuremath{^{23}\mem{Na}}}
\newcommand{\mgvi}{\ensuremath{^{24}\mem{Mg}}}
\newcommand{\mgfu}{\ensuremath{^{25}\mem{Mg}}}
\newcommand{\mgse}{\ensuremath{^{26}\mem{Mg}}}
\newcommand{\alfu}{\ensuremath{^{25}\mem{Al}}}
\newcommand{\alse}{\ensuremath{^{26}\mem{Al}}}
\newcommand{\alsi}{\ensuremath{^{27}\mem{Al}}}
\newcommand{\sisi}{\ensuremath{^{27}\mem{Si}}}
\newcommand{\siac}{\ensuremath{^{28}\mem{Si}}}
\newcommand{\sine}{\ensuremath{^{29}\mem{Si}}}
\newcommand{\sidr}{\ensuremath{^{30}\mem{Si}}}
\newcommand{\pne}{\ensuremath{^{29}\mem{P}}}
\newcommand{\pdr}{\ensuremath{^{30}\mem{P}}}
\newcommand{\pei}{\ensuremath{^{31}\mem{P}}}
\newcommand{\szw}{\ensuremath{^{32}\mem{S}}}
\newcommand{\fese}{\ensuremath{^{56}\mem{Fe}}}
\newcommand{\fesi}{\ensuremath{^{57}\mem{Fe}}}
\newcommand{\feac}{\ensuremath{^{58}\mem{Fe}}}
\newcommand{\cone}{\ensuremath{^{59}\mem{Co}}}
\newcommand{\niac}{\ensuremath{^{58}\mem{Ni}}}
\newcommand{\nine}{\ensuremath{^{59}\mem{Ni}}}
\newcommand{\nise}{\ensuremath{^{60}\mem{Ni}}}
\newcommand{\niei}{\ensuremath{^{61}\mem{Ni}}}
\newcommand{\nizw}{\ensuremath{^{62}\mem{Ni}}}
\newcommand{\nidr}{\ensuremath{^{63}\mem{Ni}}}
\newcommand{\nivi}{\ensuremath{^{64}\mem{Ni}}}
\newcommand{\cudr}{\ensuremath{^{63}\mem{Cu}}}
\newcommand{\gdr}{\ensuremath{^{63}\mem{G}}}
\newcommand{\cuvi}{\ensuremath{^{64}\mem{Cu}}}
\newcommand{\cufu}{\ensuremath{^{65}\mem{Cu}}}
\newcommand{\krfu}{\ensuremath{^{85}\mem{Kr}}}
\newcommand{\krse}{\ensuremath{^{86}\mem{Kr}}}
\newcommand{\rbse}{\ensuremath{^{86}\mem{Rb}}}
\newcommand{\rbsi}{\ensuremath{^{87}\mem{Rb}}}
\newcommand{\zrse}{\ensuremath{^{96}\mem{Zr}}}
\newcommand{\zrvi}{\ensuremath{^{94}\mem{Zr}}}
\newcommand{\zrfu}{\ensuremath{^{95}\mem{Zr}}}
\newcommand{\srac}{\ensuremath{^{88}\mem{Sr}}}
\newcommand{\iac}{\ensuremath{^{128}\mem{I}}}
\newcommand{\xeac}{\ensuremath{^{128}\mem{Xe}}}
\newcommand{\xedr}{\ensuremath{^{130}\mem{Xe}}}
\newcommand{\taac}{\ensuremath{^{180}\mem{Ta}}}
\newcommand{\csvi}{\ensuremath{^{134}\mem{Cs}}}
\newcommand{\baac}{\ensuremath{^{138}\mem{Ba}}}
\newcommand{\smei}{\ensuremath{^{151}\mem{Sm}}}
\newcommand{\blac}{\ensuremath{^{208}\mem{Pb}}}
\newcommand{\bine}{\ensuremath{^{209}\mem{Bi}}}

% 
%   units 
%
\newcommand{\msun}{\ensuremath{\, {\rm M}_\odot}}
\newcommand{\lsun}{\ensuremath{\, {\rm L}_\odot}}
\newcommand{\zsun}{\ensuremath{\, {\rm Z}_\odot}}
\newcommand{\rsun}{\ensuremath{\, {\rm R}_\odot}}
\newcommand{\dsun}{\ensuremath{\, {\rm d}_\odot}}
\newcommand{\MeV}{\ensuremath{\, \mathrm{MeV}}} 
\newcommand{\kpc}{\ensuremath{\, \mathrm{kpc}}} 
%
%   luminosities
%
\newcommand{\lumhe}{\ensuremath{L_{\rm He}}} 
\newcommand{\lumh}{\ensuremath{L_{\rm H}}} 
%
%
%   temperatures
%
\newcommand{\teight}{\ensuremath{T_{\rm 8}}}
\newcommand{\teff}{\ensuremath{T_{\rm eff}}}
\newcommand{\kelv}{\ensuremath{\,\mathrm K}}
%
%   timescales, timestep...
%
\newcommand{\tcool}{\ensuremath{\tau_{\rm cool}}}
\newcommand{\thauf}{\ensuremath{\tau_{\rm cluster}}}
\newcommand{\tagb}{\ensuremath{\tau_{\rm pWD}}}
\newcommand{\dtime}{\ensuremath{\Delta t}}
\newcommand{\years}{\ensuremath{\, \mathrm{yr}}}
%
%   masses
%
\newcommand{\mbot}{\ensuremath{M_\mem{BOT}}}
\newcommand{\mhyd}{\ensuremath{M_{\rm HYD}}}    % wasserstofffreier Kern
\newcommand{\mdup}{\ensuremath{M_{\rm dup}}}    
\newcommand{\mf}{\ensuremath{M_{\rm f}}}
\newcommand{\mg}{\ensuremath{M_{\rm G}}}
\newcommand{\mi}{\ensuremath{M_{\rm ZAMS}}}
\newcommand{\mh}{\ensuremath{M_{\rm H}}}        % Masse der Wasserstoffschicht auf WD's
\newcommand{\mheins}{\ensuremath{M_{\rm H1}}}        % M_H am 1. TP
\newcommand{\mcc}{\ensuremath{M_{\rm C}}}       % konvectiver Kern
\newcommand{\mr}{\ensuremath{M_{\rm r}}}        
\newcommand{\mhe}{\ensuremath{M_{\rm He}}}
\newcommand{\mzams}{\ensuremath{M_{\rm ZAMS}}}
%
%   velocities
%
\newcommand{\vrot}{\ensuremath{v_{\rm rot}}}

%
%   parameter
%
\newcommand{\fover}{\ensuremath{f}}
%
%   constants
%

%
%    derivatives
%

%
%       other
%
\newcommand{\mdot}{\ensuremath{\dot{M}}}
%
%
%     journals and references
%
\newcommand{\etal}{et~al.\,}
\newcommand{\etalk}{et~al.,\,}
%
%       miscalleneous
%
% arcmin, arcsec
\def\amin{{\mathaccent"0362\mathchar"070D}}
\def\asec{{\mathaccent"0362\mathchar"0722}} 
%\newcommand{\arcmin}{\hspace{-0.25em}\mbox{\,$\amin$}}    %    arcmin
%\newcommand{\arcsec}{\hspace{-0.25em}\mbox{\,$\asec$}}    %    arcsec

% equation, equation array, displaymath
\newcommand{\beq}{\begin{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\bedis}{\begin{displaymath}}
\newcommand{\edis}{\end{displaymath}}

% gradients
\newcommand{\gradad}{\ensuremath{\nabla_\mathrm{ad}}}
\newcommand{\gradrad}{\ensuremath{\nabla_\mathrm{rad}}}

\newcommand{\tenex}[2]{\ensuremath{#1 \cdot 10^{#2}}}
\newcommand{\rb}[1]{\raisebox{1.6ex}[-1.6ex]{#1}}

\newcommand{\mem}[1]{\ensuremath{\mathrm{ #1}}}

% Satzzeichen in/nach Gleichungen
\newcommand{\komma}{\mathrm{ \hspace*{0.1cm},}}
\newcommand{\punkt}{\mathrm{ \hspace*{0.1cm}.}}

%comparison operator
\newcommand{\apleq}{\ensuremath{\stackrel{<}{_\sim}}}
\newcommand{\apgeq}{\ensuremath{\stackrel{>}{_\sim}}}

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
%   other abbreviations
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
\newcommand{\dup}{dredge-up}
\newcommand{\Dup}{Dredge-up}

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
%    objects
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
\newcommand{\sak}{\mbox{V\,4334\,Sgr}}
\newcommand{\vthree}{\mbox{V\,348\,Sgr}}
\newcommand{\vsix}{\mbox{V\,605\,Aq}}

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
%    misc
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
\newcommand{\frage}{{\bf {????????}}}
\newcommand{\ov}{{\it overshoot}}
\newcommand{\diff}{{\rm d} \/}
\newcommand{\nan}{t_{\rm cluster}<t_{\rm WD}}
\newcommand{\sg}{\mmi \gg 10\msun}

\newcommand{\maov}{\alpha_c}
\newcommand{\aov}{$\alpha_c$}
\newcommand{\dov}{$d_{over}/H_p$ \/}
\newcommand{\mdov}{d_{over}/H_p }
\newcommand{\lov}{$l/H_p$}
\newcommand{\mlov}{l/H_p}
\newcommand{\hp}{\ensuremath{H_\mem{p}}}
\newcommand{\lmh}{$\log{M_{\rm H}/M_{\ast}}$}
\newcommand{\mlmh}{\log{M_{\rm H}/M_{\ast}}}
\newcommand{\lmhe}{\ensuremath{\log{M_{\rm He}/M_{\ast}}}}
\newcommand{\fst}{\ensuremath{1^\mem{st}}}
\newcommand{\third}{\ensuremath{3^\mem{rd}}}
\newcommand{\rarr}{\ensuremath{\rightarrow}}
\newcommand{\larr}{\ensuremath{\leftarrow}}
\newcommand{\lra}{\ensuremath{\leftrightarrow}}


\newcommand{\tenh}[2]{\ensuremath{#1\times10^#2}}

